OpenFed: A Comprehensive and Versatile Open-Source Federated Learning Framework

Recent developments in Artificial Intelligence techniques have enabled their successful application across a spectrum of commercial and industrial settings. However, these techniques require large volumes of data to be aggregated in a centralized manner, forestalling their applicability to scenarios wherein the data is sensitive or the cost of data transmission is prohibitive. Federated Learning alleviates these problems by decentralizing model training, thereby removing the need for data transfer and aggregation. To advance the adoption of Federated Learning, more research and development needs to be conducted to address some important open questions. In this work, we propose OpenFed, an open-source software framework for end-to-end Federated Learning. OpenFed reduces the barrier to entry for both researchers and downstream users of Federated Learning by the targeted removal of existing pain points. For researchers, OpenFed provides a framework wherein new methods can be easily implemented and fairly evaluated against an extensive suite of benchmarks. For downstream users, OpenFed allows Federated Learning to be plugged and play within different subject-matter contexts, removing the need for deep expertise in Federated Learning.

==> fig/cmp.tex <==
\begin{table}[!ht]
  \caption{Comparison between the OpenFed and existing FL frameworks.}
  \label{tab:platform-summary}
\begin{tabular}{cl|cccccccccc}
                                                     &                                          & CrypTen & FATE    & PaddleFL & PySyft  & FedML   & FFL-ERL & LEAF    & TensorIO & TFF     & OpenFed \\ \hline
    \multirow{3}{*}{Diverse computing paradigms}     & Standalone simulation                    &         & $\surd$ & $\surd$  & $\surd$ & $\surd$ &         & $\surd$ &          & $\surd$ & $\surd$ \\
                                                     & Distributed computing                    & $\surd$ & $\surd$ & $\surd$  & $\surd$ & $\surd$ &         &         &          & $\surd$ & $\surd$ \\
                                                     & On-device training                       &         &         &          &         & $\surd$ & $\surd$ &         & $\surd$  &         & $\surd$ \\ \hline
    \multirow{4}{*}{Flexible and generic API design} & Message flow                             &         &         &          &         & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & Customize heterogeneous data distribution &         &         &          &         &         &         & $\surd$ &          &         & $\surd$ \\
                                                     & Unified paradigms                        &         & $\surd$ & $\surd$  & $\surd$ &         &         &         &          & $\surd$ & $\surd$ \\
                                                     & Third-party supports                     &         &         &          & $\surd$ &         &         &         &          &         & $\surd$ \\ \hline
    \multirow{5}{*}{Topology customization}          & Split                                    &         &         & $\surd$  & $\surd$ & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & Vertical                                 &         & $\surd$ & $\surd$  &         & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & Hierarchical                             &         &         &          &         &         &         &         &          &         & $\surd$ \\
                                                     & Decentralized                            &         &         &          &         & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & Centralized                              & $\surd$ & $\surd$ & $\surd$  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$  & $\surd$ & $\surd$ \\ \hline
    \multirow{4}{*}{Federated optimizer}             & Aggregation customization                &         &         &          &         & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & Gradient accumulation                     &         &         &          &         &         &         &         &          &         & $\surd$ \\
                                                     & Parameter penalization                   &         &         &          &         & $\surd$ &         &         &          &         & $\surd$ \\
                                                     & States synchronization                   &         &         &          &         &         &         &         &          &         & $\surd$ \\ \hline
    \multirow{4}{*}{Benchmarks}                      & Computer vision                          &         & $\surd$ & $\surd$  & $\surd$ & $\surd$ &         & $\surd$ & $\surd$  & $\surd$ & $\surd$ \\
                                                     & Natural language processing              &         & $\surd$ & $\surd$  &         & $\surd$ &         & $\surd$ &          & $\surd$ & $\surd$ \\
                                                     & Reinforcement learning                   &         &         &          &         &         &         &         &          &         & $\surd$ \\
                                                     & Medical analysis                         &         &         &          & $\surd$ &         &         &         &          &         & $\surd$
    \end{tabular}
\end{table}

==> fig/tab.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/tab.pdf}
    \caption{Comparison between OpenFed and existing FL frameworks.}
    \label{tab:platform-summary}
\end{figure*}


